Prediction of a T-cell/MHC-I-based immune profile for colorectal liver metastases from CT images using ensemble learning

Colorectal cancer liver metastases (CLM) are the most common type of distant metastases originating from the abdomen and are characterized by a high recurrence rate after curative resection. It has been previously reported that CLM presenting a low cluster of differentiation 3 (CD3) positive T-cell infiltration density concurrent with a high major histocompatibility complex class I (MHC-I) expression were associated with poor clinical outcomes. In this study, we attempt to noninvasively predict whether a CLM exhibit the CD3LowMHCHigh immunological profile using preoperative CT images. To this end, we propose an ensemble network combining multiple Attentive Interpretable Tabular learning (TabNet) models, trained using CT-derived radiomic features. A total of 160 CLM were included in this study and randomly divided between a training set (n=130) and a hold-out test set (n=30). The proposed model yielded good prediction performance on the test set with an accuracy of 70.0% [95% confidence interval 53.6%-86.4%] and an area under the curve of 69.4% [52.9%-85.9%]. It also outperformed other off-the-shelf machine learning models. We finally demonstrated that the predicted immune profile was associated with a shorter disease-specific survival (p = .023) and time-to-recurrence (p = .020), showing the value of assessing the immune response.

==> backup.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{c c c c c c}
         Toxicity & Input & Fraction & Balanced accuracy (\%) & Specificity (\%) & Sensitivity (\%) \\
         \hline\hline \\
         \multirow{9}{*}{Necrosis} & Clinical + deformation & Week 7 & & & \\
         & Clinical + deformation & Week 6 & & & \\
         & Clinical + deformation & Week 5 & & & \\
         & Clinical + deformation & Week 4 & & & \\
         & Clinical + deformation & Week 3 & & & \\
         & Clinical + deformation & Week 2 & 85.8 & 93.3 & 78.2 \\
         & Clinical + deformation & Week 1 & & & \\
         & Clinical + deformation & Treatment start & & & \\
         & Clinical & \textit{N/A} & 75.7 & 86.7 & 75.4 \\
         \hline \\
         \multirow{2}{*}{Hospitalization} & Clinical + deformation & Week 7 & & & \\
         & Clinical + deformation & Week 6 & & & \\
         & Clinical + deformation & Week 5 & & & \\
         & Clinical + deformation & Week 4 & & & \\
         & Clinical + deformation & Week 3 & & & \\
         & Clinical + deformation & Week 2 & 75.3 & 83.1 & 67.4 \\
         & Clinical + deformation & Week 1 & & & \\
         & Clinical + deformation & Treatment start & & & \\
         & Clinical & \textit{N/A} & 63.1 & 49.3 & 63.6 \\
         \hline \\
         \multirow{2}{*}{Reactive TNG} & Clinical + deformation & Week 7 & & & \\
         & Clinical + deformation & Week 6 & & & \\
         & Clinical + deformation & Week 5 & & & \\
         & Clinical + deformation & Week 4 & & & \\
         & Clinical + deformation & Week 3 & & & \\
         & Clinical + deformation & Week 2 & 69.1 & 64.3 & 73.9 \\
         & Clinical + deformation & Week 1 & & & \\
         & Clinical + deformation & Treatment start & & & \\
         & Clinical & \textit{N/A} & 57.2 & 64.6 & 55.4 \\
         \hline \\
    \end{tabular}
    \caption{
        Classification performance for each toxicity outcome against different inputs.
        The baseline model contains only the feed-forward path for classifying clinical data.
        Models with deformation inputs in the form of Jacobian determinant matrix between the baseline CT and the daily CBCT add an additional ResNet-like\cite{resnet} 3D convolutional branch before the classification layers.
        Deformation are computed using on the CBCT acquired before the last fraction of the corresponding week is delivered, with using 5 days per work week.}
    \label{tab:benchmark}
\end{table*}

\begin{figure}[htb]
    \begin{minipage}[b]{1.0\linewidth}
      \centering
      \centerline{\includegraphics[width=8.5cm]{VoxelMorph.jpg}}
      \centerline{(a) Result 1}\medskip
    \end{minipage}
    \caption{
        Registration model based on the VoxelMorph architecture.
        Training was performed between either the planning CT and CBCT\textsubscript{0} or between CBCT\textsubscript{0} and CBCT\textsubscript{t}.
        The final DVF was obtained between the planning CT registered to CBCT\textsubscript{0} and the target CBCT\textsubscript{t} from which the Jacobian determinant matrix was computed.}
    \label{fig:registration}
\end{figure}
%\vfill
%\pagebreak

\begin{figure}[htb]
    \begin{minipage}[b]{1.0\linewidth}
      \centering
      \centerline{\includegraphics[width=8.5cm]{ResNet.jpg}}
      \centerline{(a) Result 1}\medskip
    \end{minipage}
    \caption{
        Multi-branch classification model based on ResNet50.
        Two branch types were defined with their own set of shared weights: a CBCT feature extractor, and a Jacobian deformation analysis branch.
        Each had the option of additional masking based on OAR or tumor segmentation.
        A third fully connected input branch processed clinical data.
        The latent embedding of each input modality were concatenated before final classification into one of three radiotherapy toxicity outcome: necrosis, hospitalization and TNG.}
    \label{fig:classification}
\end{figure}
%\vfill
%\pagebreak
